Another super-dense sub-Neptune in K2-182 b and refined mass measurements for K2-199 b and c

We combine multiple campaigns of K2 photometry with precision radial velocity measurements from Keck-HIRES to measure the masses of three sub-Neptune-size planets. We confirm the planetary nature of the massive sub-Neptune K2-182 b ($P_\mathrm{b}= 4.7$ days, $R_\mathrm{b} = 2.69$ $R_\oplus$) and derive refined parameters for K2-199 b and c ($P_\mathrm{b} = 3.2$ days, $R_\mathrm{b} = 1.73$ $R_\oplus$, and $P_\mathrm{c} = 7.4$ days, $R_\mathrm{c} = 2.85$ $R_\oplus$). These planets provide valuable data points in the mass-radius plane, especially as TESS continues to reveal an increasingly diverse sample of sub-Neptunes. K2-182 (EPIC 211359660) is a moderately bright ($V = 12.0$ mag) early-K dwarf observed during K2 campaigns 5 and 18. We find K2-182 b is potentially one of the densest sub-Neptunes known to date ($20 \pm 5$ $M_\oplus$ and $5.6 \pm 1.4$ g cm$^{-3}$). K2-199 (EPIC 212779596; $V = 12.3$ mag) is a K5V dwarf observed in K2 campaigns 6 and 17 which hosts two recently-confirmed planets. We refine the orbital and planetary parameters for K2-199 b and c by modeling both campaigns of K2 photometry and adding 12 Keck-HIRES measurements to the existing radial velocity data set ($N$ = 33). We find K2-199 b is likely rocky, at $6.9 \pm 1.8$ $M_\oplus$ and $7.2^{+2.1}_{-2.0}$ g cm$^{-3}$. K2-199 c has an intermediate density at $12.4 \pm 2.3$ $M_\oplus$ and $2.9^{+0.7}_{-0.6}$ g cm$^{-3}$. We contextualize these planets on the mass-radius plane, discuss a small but intriguing population of "super-dense" sub-Neptunes ($R_\mathrm{p} < 3$ $R_\oplus$, $M_\mathrm{p} > 20$ $M_\oplus$), and consider our prospects for the planets' atmospheric characterization.

==> k2-199_rvs_FULL.tex <==
\begin{deluxetable}{lrrrrc}
\tablecaption{K2-199 radial velocities \label{tab:k2-199_rvs_FULL}}
\tablehead{
\colhead{Time} & 
\colhead{RV} & 
\colhead{RV Unc.} &
\colhead{Inst.} \\
\colhead{(JD)} & 
\colhead{(m s$^{-1}$)} & 
\colhead{(m s$^{-1}$)} & 
\colhead{}
}
\startdata
2457562.85035 & -2.17 & 1.31 & HIRES \\
2457585.84130 & -6.14 & 1.50 & HIRES \\
2457586.82765 & -15.29 & 1.39 & HIRES \\
2457587.84055 & -1.05 & 1.51 & HIRES \\
2457600.80170 & -19.12 & 1.63 & HIRES \\
2457760.13919 & 1.92 & 1.99 & HIRES \\
2457789.10883 & 5.68 & 1.64 & HIRES \\
2457790.10369 & -7.51 & 1.49 & HIRES \\
2457791.09856 & -5.49 & 1.63 & HIRES \\
2457793.10850 & -6.51 & 1.67 & HIRES \\
2457794.13640 & -4.56 & 1.43 & HIRES \\
2457795.01046 & 11.73 & 1.69 & HIRES \\
2457807.07494 & -3.82 & 1.85 & HIRES \\
2457830.11149 & -9.85 & 1.75 & HIRES \\
2457831.06501 & -4.56 & 1.66 & HIRES \\
2457852.99056 & -3.87 & 1.57 & HIRES \\
2457887.01304 & -7.24 & 1.75 & HIRES \\
2457906.99131 & -2.53 & 1.84 & HIRES \\
2457912.94485 & 1.35 & 1.93 & HIRES \\
2457925.91160 & -6.44 & 1.84 & HIRES \\
2457926.91550 & 1.35 & 1.56 & HIRES \\
2457932.85055 & -12.10 & 1.74 & HIRES \\
2457933.78112 & 0.70 & 1.55 & HIRES \\
2457934.78185 & -0.92 & 1.58 & HIRES \\
2457939.84182 & -0.46 & 1.94 & HIRES \\
2457940.87896 & 5.91 & 1.75 & HIRES \\
2457971.78716 & 1.73 & 1.83 & HIRES \\
2457988.74362 & 13.64 & 2.29 & HIRES \\
2458114.14627 & -1.09 & 1.72 & HIRES \\
2458125.10424 & -3.04 & 1.55 & HIRES \\
2458150.04042 & 7.98 & 1.57 & HIRES \\
2458151.03592 & 5.57 & 1.85 & HIRES \\
2458195.01417 & 2.35 & 1.67 & HIRES \\
2458533.11808 & 2.39 & 1.82 & HIRES \\
2458560.06257 & -8.44 & 1.73 & HIRES \\
2458568.90252 & 6.03 & 1.60 & HIRES \\
2458569.91236 & 6.26 & 1.72 & HIRES \\
2458591.97627 & 0.24 & 1.76 & HIRES \\
2458595.86178 & -4.35 & 1.60 & HIRES \\
2458615.86603 & -5.36 & 1.89 & HIRES \\
2458616.85860 & -3.86 & 1.82 & HIRES \\
2458617.85161 & -2.68 & 1.74 & HIRES \\
2458627.86391 & -2.16 & 1.53 & HIRES \\
2458632.84003 & -7.41 & 1.71 & HIRES \\
2458633.85508 & -5.40 & 1.47 & HIRES \\
\enddata
\tablecomments{The combined dataset ($N = 45$) of K2-199 RVs from this work and \nasakeyproj. This table is available online in machine readable format. The RV uncertainties listed here are added in quadrature with an instrumental parameter for RV jitter, $\sigma_j =  4.14$ \mps, that was fit to the data.
}
\end{deluxetable}
